Rate-Resolved Text Evaluation with Masked Diffusion Language Models

A single evaluation score can rank generation systems but rarely reveals what failed. We propose rate-resolved text evaluation, which turns the masking rate of masked diffusion language models into a diagnostic axis. By reconstructing text under different fractions of masked tokens, one diffusion score becomes a vector of band-conditioned scores that reflect reconstruction difficulty at varying levels of visible context. On SummEval, preserving this rate structure yields complementary signal: the best masking-rate band improves fusion with autoregressive likelihood over a collapsed diffusion scalar, survives a sample-shuffle control that breaks rate ordering, and adds residual signal to a fixed prompted judge. A second diffusion model reproduces the effect more weakly. On WMT MQM zh-en, roundtrip mask-and-reconstruct probing produces a tunable localization curve in which ranking-oriented AUROC and span-detection F1 peak at different masking rates. Factuality benchmarks bound the interpretation: band semantics are model- and task-dependent, so each application requires empirical validation.

==> tables/core_results.tex <==
% Required packages:
% \usepackage{booktabs}
% \usepackage{array}

\newcommand{\evidencecell}[3]{%
\begin{minipage}[t]{\linewidth}
\raggedright
\textbf{#1}\par
{\footnotesize\emph{#2}}\par
\vspace{4pt}
{\footnotesize #3}
\end{minipage}
}

\begin{table*}[!t]
\centering
\small
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{1.0}

\begin{tabular}{
@{}
p{0.29\textwidth}
@{\hspace{0.055\textwidth}}
p{0.29\textwidth}
@{\hspace{0.055\textwidth}}
p{0.29\textwidth}
@{}
}

\toprule
\multicolumn{3}{@{}l}{\textbf{Main evidence}} \\
\midrule

\evidencecell
{Rate structure}
{SummEval control}
{AR+band $>$ AR+scalar:
$\Delta\rho=\mathbf{+0.0185}$,
$p=\mathbf{0.0015}$.}
&
\evidencecell
{Judge complementarity}
{SummEval primary}
{Judge $0.3065 \rightarrow \mathbf{0.3454}$;
judge+AR+diff. reaches $\mathbf{0.3636}$.}
&
\evidencecell
{Tunable localization}
{WMT MQM primary}
{AUROC $\mathbf{0.6705}$ at $s=0.5$;
major F1 $\mathbf{0.3464}$ at $s=0.3$.}
\\

\addlinespace[11pt]
\midrule
\multicolumn{3}{@{}l}{\textbf{Controls and scope}} \\
\midrule

\evidencecell
{Baseline control}
{WMT MQM}
{XLM-R-XXL AUROC $0.6236 < \mathbf{0.6705}$;
AR wins pooled F1, $\mathbf{0.2636} > 0.2311$.}
&
\evidencecell
{Model replication}
{SummEval}
{Dream gives a weaker but aligned gain:
$\rho=\mathbf{0.2638}$.}
&
\evidencecell
{Semantic boundary}
{FRANK / FActScore}
{Controlled effects shrink or shift:
FRANK $\approx 0.08$; FActScore $0.215$.}
\\

\bottomrule
\end{tabular}

\caption{
Empirical support for rate-resolved evaluation. Main results are shown in the upper row, with controls and scope checks shown below.
}
\label{tab:core-results}
\end{table*}
